Self-Taught Agentic Long Context Understanding

Answering complex, long-context questions remains a major challenge for large language models (LLMs) as it requires effective question clarifications and context retrieval. We propose Agentic Long-Context Understanding (AgenticLU), a framework designed to enhance an LLM's understanding of such queries by integrating targeted self-clarification with contextual grounding within an agentic workflow. At the core of AgenticLU is Chain-of-Clarifications (CoC), where models refine their understanding through self-generated clarification questions and corresponding contextual groundings. By scaling inference as a tree search where each node represents a CoC step, we achieve 97.8% answer recall on NarrativeQA with a search depth of up to three and a branching factor of eight. To amortize the high cost of this search process to training, we leverage the preference pairs for each step obtained by the CoC workflow and perform two-stage model finetuning: (1) supervised finetuning to learn effective decomposition strategies, and (2) direct preference optimization to enhance reasoning quality. This enables AgenticLU models to generate clarifications and retrieve relevant context effectively and efficiently in a single inference pass. Extensive experiments across seven long-context tasks demonstrate that AgenticLU significantly outperforms state-of-the-art prompting methods and specialized long-context LLMs, achieving robust multi-hop reasoning while sustaining consistent performance as context length grows.

==> img/fig_datastat.tex <==
\begin{figure}[t!]
    \begin{center}
    \includegraphics[width=0.9\columnwidth , keepaspectratio]{img/datastat.pdf}
    \end{center}
    \caption{\textbf{Most questions can be answered with up to three rounds of clarifications.} 
    A single round of clarification suffices for the majority of questions (92\%), with a smaller fraction requiring two or three additional clarifications. 
    We cap inference-time clarifications at three rounds to strike a balance between coverage (solving 97.4\% of questions) and computational cost.}
    \label{fig:dataset_stat}
\end{figure}

==> img/pipeline_figure_small.tex <==
\begin{figure}[t!]
    \begin{center}
    \includegraphics[width=\columnwidth , keepaspectratio]{img/agentlu_small.pdf}
    \end{center}
    \caption{\textbf{An overview of the agentic workflow for tackling long-context tasks.} The model first raises or identifies a clarifying question (1), locates relevant context (2), clarifies its own reasoning (3), and finally provides an answer (4). The reasoning process can be multi-round depending on the complexity of the tasks at hand.
    % \jingbo{this figure makes me feel like an iterative process.}
    }
    \label{fig:pipeline_small}
\end{figure}

==> tab/main_table.tex <==
\begin{table*}[ht]
  \centering
  \caption{Performance on \texttt{infbench\_qa}, \texttt{infbench\_choice}, and \texttt{narrativeqa} Across Context Lengths}
  \label{tab:main_table}
  \resizebox{\textwidth}{!}{
  \begin{tabular}{l *{15}{c}}
    \toprule
                      & \multicolumn{5}{c}{infbench\_qa} & \multicolumn{5}{c}{infbench\_choice} & \multicolumn{5}{c}{narrativeqa} \\
    \cmidrule(lr){2-6} \cmidrule(lr){7-11} \cmidrule(lr){12-16}
    Model             & 8K   & 16K  & 32K  & 64K  & 128K & 8K   & 16K  & 32K  & 64K  & 128K & 8K   & 16K  & 32K  & 64K  & 128K \\
    \midrule
    Llama3.1 8B       & 17 & 31 & 36 & 40 & 48 & 9  & 12 & 24 & 39 & 55 & 15 & 19 & 27 & 35 & 38 \\
    Qwen-14B          & 21 & 34 & 39 & 47 & 55 & 29 & 29 & 37 & 47 & 53 & 22 & 31 & 37 & 52 & 57 \\
    ProLong-8B        & 16 & 31 & 29 & 31 & 45 & 22 & 27 & 37 & 48 & 58 & 18 & 27 & --   & --   & 42 \\
    AgenticLU-8B-SFT   & --   & --   & --   & --   & 55 & --   & --   & --   & --   & 58 & --   & --   & --   & --   & 60 \\
    \bottomrule
  \end{tabular}
  }
\end{table*}

==> tab/prompting_table.tex <==
\begin{table*}[ht]
  \centering
  \caption{Performance on infbench\_qa, infbench\_choice, and narrativeqa Across Context Lengths}
  \label{tab:prompting_table}
  \resizebox{\textwidth}{!}{
  \begin{tabular}{l *{15}{c}}
    \toprule
    & \multicolumn{5}{c}{infbench\_qa} & \multicolumn{5}{c}{infbench\_choice} & \multicolumn{5}{c}{narrativeqa} \\
    \cmidrule(lr){2-6} \cmidrule(lr){7-11} \cmidrule(lr){12-16}
    Model            & 8K   & 16K  & 32K  & 64K  & 128K & 8K   & 16K  & 32K  & 64K  & 128K & 8K   & 16K  & 32K  & 64K  & 128K \\
    \midrule
    Llama3.1 8B      & 17 & 31 & 36 & 40 & 48 & 9  & 12 & 24 & 39 & 55 & 15 & 19 & 27 & 35 & 38 \\
    -StepbyStep      & 21 & 36 & 36 & 45 & 43 & 15 & 13 & 41 & 41 & 44 & 23 & 30 & 36 & 51 & 43 \\
    -Plan\&Solve     & 17 & 26 & 32 & 41 & 40 & 27 & 15 & 48 & 55 & 58 & 22 & 25 & 38 & 41 & 39 \\
    -Fact\&Reflect   & 19 & 30 & 40 & 42 & 37 & 20 & 14 & 38 & 51 & 56 & 21 & 35 & 37 & 42 & 46 \\
    LongRAG          & --   & --   & --   & --   & --   & --   & --   & --   & --   & --   & --   & --   & --   & --   & --   \\
    AgenticLU        & --   & --   & --   & --   & 62 & --   & --   & --   & --   & 67 & --   & --   & --   & --   & 57 \\
    \bottomrule
  \end{tabular}
  }
\end{table*}
